Cyclic Descents for General Skew Tableaux

A cyclic descent function on standard Young tableaux of size $n$ is a function that restricts to the usual descent function when $n$ is omitted, such that the number of standard Young tableaux of given shape with cyclic descent set $D\subset[n]$ is invariant under any modulo $n$ shift of $D$. The notion of cyclic descent was first studied for rectangles by Rhoades, and then generalized to certain families of skew shapes by Adin, Elizalde, and Roichman. Adin, Reiner, and Roichman proved that a skew shape has a cyclic descent map if and only if it is not a connected ribbon. Unfortunately, their proof is nonconstructive; until now, explicit cyclic descent maps are known only for small families of shapes. In this paper, we construct an explicit cyclic descent map for all shapes where this is possible. We thus provide a constructive proof of Adin, Reiner, and Roichman's result. Our construction of a cyclic descent map generalizes many of the constructions in the literature.

==> src/special-cases-abridged.tex <==
\section{Special Cases}\label{sec:special-cases}

\subimport{\spcasesAbr}{top}
\subimport{\spcasesAbr}{rectangles}
\subimport{\spcasesAbr}{hook-plus-internal}
\subimport{\spcasesAbr}{two-row}
\subimport{\spcasesAbr}{disconnected-northeast}


==> src/special-cases-abridged/disconnected-northeast.tex <==
\subsection{Young Diagram with Disconnected Northeast Cell}

The following construction is due to Elizalde and Roichman.

\begin{thm}\cite[Proposition 5.3]{ER}\label{thm:er}
    Let $\skewshape$ consist of a Young diagram of size $n-1$ and a disconnected northeast cell.
    For $T\in \SYT(\skewshape)$, let $n\in \cDes(T)$ if and only if one of the following holds.
    \begin{enumerate}
        \item $n$ is in the disconnected cell.
        \item $d\neq n$ is in the disconnected cell and $n-d\in \Des(\jdt(-d+T))$
    \end{enumerate}
    Moreover, define $\phi'$ by
    \begin{equation*}
        \phi'(T) = \jdt(1+d+\jdt(-d+T)).
    \end{equation*}
    Then $(\cDes',\phi')$ is a cyclic descent map.
\end{thm}

This cyclic descent map is \textit{not} a special case of $(\cDes,\phi)$.
As a counterexample, let
\begin{equation*}
    T = \young(:::1,235,46).
\end{equation*}
Then
\begin{equation*}
    \phi T = \young(:::2,134,56)
    \quad
    \text{and}
    \quad
    \phi' T = \young(:::2,146,35),
\end{equation*}
so $\phi T \neq \phi' T$.
Moreover, $\cDes(\phi T) = \{2,4,6\}$, while $\cDes'(\phi T) = \{2,4\}$.


==> src/special-cases-abridged/hook-plus-internal.tex <==
\subsection{Hook Plus Internal Cell}

Let $\lambda = (n-k, 2, 1^{k-2})$ and $\mu = ()$.
The following construction is due to Adin, Elizalde, and Roichman.

\begin{defn}\cite[Corollary 4.8]{AER}\label{defn:hook-internal-cdes}
For $T\in \SYT(\skewshape)$,
let $n\in \cDes'(T)$ if and only if $\pos_T(T_{2,2}-1)$ is in the first column of $T$.
\end{defn}

This construction is different from the others in that it constructs $\psi = \phi'^{-1}$ instead of $\phi'$.
\begin{defn}\cite[Definition 4.13]{AER}\label{defn:hook-internal-phi}
    For $T\in \SYT(\skewshape)$, define $\psi T$ as follows.
    \begin{itemize}
        \item If $1\not\in \Des(T)$, let the first row of $\psi T$ have entries $[n]\setminus \cDes'(T)$,
        in increasing order from west to east, where $\cDes'(T)$ is defined in Definition~\ref{defn:hook-internal-cdes}.
        Let $(\psi T)_{2,2}$ be defined as follows, depending on the location of $\pos_T(T_{2,2}-1)$.
        \begin{enumerate}[label=(\alph*)]
            \item If $\pos_T(T_{2,2}-1)$ is in the first row of $T$, $(\psi T)_{2,2}=T_{2,2}-1$.
            \item If $\pos_T(T_{2,2}-1)$ is in the first column of $T$ and not the southernmost entry $(k,1)$,
            and $a$ is the entry in its southern neighbor, $(\psi T)_{2,2}=a-1$.
            \item If $\pos_T(T_{2,2}-1) = (k,1)$, $(\psi T)_{2,2}=n$.
        \end{enumerate}
        The remaining entries are in the first column of $T$, in increasing order from north to south.
        \item If $1\in \Des(T)$, let $\psi T = (\psi T^{\tra})^{\tra}$, reducing to the previous case.
    \end{itemize}
\end{defn}

\begin{thm}\label{thm:aer-hook-internal}\cite[Theorem 1.11]{AER}
    Let $\cDes'$ be defined by Definition~\ref{defn:hook-internal-cdes}, and let $\phi' = \psi^{-1}$,
    where $\psi$ is defined by Definition~\ref{defn:hook-internal-phi}.
    Then $(\cDes',\phi')$ is a cyclic descent map.
\end{thm}

The cyclic descent map $(\cDes', \phi')$, defined in Theorem~\ref{thm:aer-hook-internal},
coincides with the $(\cDes, \phi)$ defined in Theorem~\ref{thm:main}.


==> src/special-cases-abridged/rectangles.tex <==
\subsection{Rectangles and Strips}

Recall this result by Rhoades, stated in Section~\ref{sec:intro}.
\begin{repthm}{thm:rhoades}\cite[Lemma 3.3]{Rho}
    Let $\skewshape$ be a rectangular Young diagram with length and width both larger than 1.
    Let $\phi' = \pro$, and let $n\in \cDes'(T)$ if and only if $n-1 \in \Des(\dem T)$.
    Then $(\cDes', \phi')$ is a cyclic descent map.
\end{repthm}

Adin, Elizalde, and Roichman give an analogous construction for \vocab{strips},
skew shapes with more than one connected component
whose connected components are all single-row or single-column rectangles.
\begin{thm}\label{thm:aer-strip}\cite[Proposition 3.3]{AER}
    Let $\skewshape$ be a strip.
    Let $\phi' = \pro$, and let $n\in \cDes'(T)$ if and only if $n-1 \in \Des(\dem T)$.
    Then $(\cDes', \phi')$ is a cyclic descent map.
\end{thm}

The cyclic descent map $(\cDes', \phi')$,
defined in Theorems~\ref{thm:rhoades} and \ref{thm:aer-strip},
coincides with the $(\cDes, \phi)$ defined in Theorem~\ref{thm:main}.

In fact, it can be shown that $(\phi, \cDes)$ and $(\phi', \cDes')$
are the same for a family of $\skewshape$ including both rectangles and strips.
\begin{cor}
	In any skew shape $\skewshape$ whose connected components are all rectangles,
	$(\phi, \cDes)$ and $(\phi', \cDes')$ are the same.
\end{cor}


==> src/special-cases-abridged/top.tex <==
In this section we review some of the literature
for cyclic descents of skew tableaux.
We will state which of the constructions in the literature
are special cases of Theorem~\ref{thm:main}.
The proofs that these constructions coincide with the construction in
Theorem~\ref{thm:main} are sometimes complex.
Thus, we omit the proofs here;
the proofs can be found in the arXiv version of this paper,
at \href{https://arxiv.org/abs/1808.04918}{arXiv:1808.04918}.

First, let us introduce the relevant definitions from the literature.

For a (not necessarily standard) tableau $T$ of shape $\skewshape$ and integer $a$,
let $a+T$ be the tableau obtained by adding $a$ to each entry of $T$ and taking entries modulo $n$.

Where appropriate, we will also name cells by their coordinates.
Thus, $(x,y)$ is the cell in the $x^{\text{th}}$ row and $y^{\text{th}}$ column of $\skewshape$
where $(1,1)$ is the shared northwest corner of $\lambda$ and $\mu$.
Let $T_{x,y}$ denote the entry of $T$ in cell $(x,y)$.

The \vocab{generalized jeu de taquin} operator $\jdt$ \cite[Definition 2.3]{AER} acts on a tableau $T$ as follows.
While $T$ is not standard, apply the following operation to $T$:
find the minimal entry $i$ such that $i$ is not smaller than both its northern and western neighbors,
and swap $i$ with the larger of these neighbors.

\begin{ex}
    Below is one action of $\jdt$ on a nonstandard tableau.
    \begin{equation*}
        \young(342,51)
        \quad \mapsto \quad
        \young(342,15)
        \quad \mapsto \quad
        \young(142,35)
        \quad \mapsto \quad
        \young(124,35).
    \end{equation*}
\end{ex}
\begin{rem}
    For all $T\in \SYT(\skewshape)$,
    \begin{equation*}
    \pro(T) = \jdt(1+T)
    \quad
    \text{and}
    \quad
    \dem(T) = \jdt(-1+T).
    \end{equation*}
\end{rem}

Throughout this section, we adopt the following notational convention.
We use $(\cDes, \phi)$ to denote the cyclic descent map given
in Theorem~\ref{thm:main},
and $(\cDes',\phi')$ to denote the cyclic descent maps from the literature
that we are comparing to $(\cDes, \phi)$.


==> src/special-cases-abridged/two-row.tex <==
\subsection{Two-Row Straight Shapes}

Let $\lambda = (n-k,k)$ with $2\le k\le n/2$ and $\mu = ()$.
The following construction is due to Adin, Elizalde, and Roichman.

\begin{defn}\label{defn:two-row-cdes}\cite[Definition 1.12]{AER}
    For $T\in \SYT(\skewshape)$,
    let $n\in \cDes'(T)$ if and only if both of the following conditions hold.
    \begin{enumerate}
        \item $T_{2,k} = T_{2,k-1}+1$.
        \item For every $1<i<k$, $T_{2,i-1} > T_{1,i}$.
    \end{enumerate}
\end{defn}

By a slight abuse of notation, let $1+T_{\le x}$ denote the tableau obtained by
adding $1$ modulo $x$ to the entries $1,\ldots,x$ in $T$,
and leaving the remaining entries unchanged.

\begin{defn}\label{defn:two-row-phi}\cite[Definition 5.13]{AER}
    For $T\in \SYT(\skewshape)$, define $\phi' T$ as follows.
    \begin{enumerate}
        \item If $T_{2,k} = T_{2,k-1}+1$, let $\phi' T = \jdt(1+T_{\le x})$, where $x=T_{2,k}$.
        \item Otherwise:
        \begin{enumerate}
            \item If $n$ is in the first row of $T$, let $\phi' T = \pro(T)$.
            \item If $n$ is in the second row of $T$,
            let $\phi' T$ be the tableau obtained from $1+T$ as follows:
            switch $1$ with $y+1$, where $y$ is the entry immediately to the west of $1$, and then apply $\jdt$.
        \end{enumerate}
    \end{enumerate}
\end{defn}

\begin{thm}\label{thm:aer-two-row}\cite[Theorem 1.14]{AER}
    The $(\cDes',\phi')$ defined by Definitions~\ref{defn:two-row-cdes}
    and \ref{defn:two-row-phi} is a cyclic descent map.
\end{thm}

The cyclic descent map $(\cDes', \phi')$
defined in Theorem~\ref{thm:aer-two-row}
coincides with the $(\cDes, \phi)$ defined in Theorem~\ref{thm:main}.

